Digital Divide and Social Dilemma of Privacy Preservation

While digital divide studies primarily focused on access to information and communications technology (ICT) in the past, its influence on other associated dimensions such as privacy is becoming critical with a far-reaching impact on the people and society. For example, the various levels of government legislation and compliance on information privacy worldwide have created a new era of digital divide in the privacy preservation domain. In this article, the concept "digital privacy divide (DPD)" is introduced to describe the perceived gap in the privacy preservation of individuals based on the geopolitical location of different countries. To better understand the DPD phenomenon, we created an online questionnaire and collected answers from more than 700 respondents from four different countries (the United States, Germany, Bangladesh, and India) who come from two distinct cultural orientations as per Hofstede's individualist vs. collectivist society. However, our results revealed some interesting findings. DPD does not depend on Hofstede's cultural orientation of the countries. For example, individuals residing in Germany and Bangladesh share similar privacy concerns, while there is a significant similarity among individuals residing in the United States and India. Moreover, while most respondents acknowledge the importance of privacy legislation to protect their digital privacy, they do not mind their governments to allow domestic companies and organizations collecting personal data on individuals residing outside their countries, if there are economic, employment, and crime prevention benefits. These results suggest a social dilemma in the perceived privacy preservation, which could be dependent on many other contextual factors beyond government legislation and countries' cultural orientation.

==> source/results.tex <==
\section{Closing the Digital Privacy Divide}\label{sec:sec_4}

